Low-Quality Training Data Only? A Robust Framework for Detecting Encrypted Malicious Network Traffic

Machine learning (ML) is promising in accurately detecting malicious flows in encrypted network traffic; however, it is challenging to collect a training dataset that contains a sufficient amount of encrypted malicious data with correct labels. When ML models are trained with low-quality training data, they suffer degraded performance. In this paper, we aim at addressing a real-world low-quality training dataset problem, namely, detecting encrypted malicious traffic generated by continuously evolving malware. We develop RAPIER that fully utilizes different distributions of normal and malicious traffic data in the feature space, where normal data is tightly distributed in a certain area and the malicious data is scattered over the entire feature space to augment training data for model training. RAPIER includes two pre-processing modules to convert traffic into feature vectors and correct label noises. We evaluate our system on two public datasets and one combined dataset. With 1000 samples and 45% noises from each dataset, our system achieves the F1 scores of 0.770, 0.776, and 0.855, respectively, achieving average improvements of 352.6%, 284.3%, and 214.9% over the existing methods, respectively. Furthermore, We evaluate RAPIER with a real-world dataset obtained from a security enterprise. RAPIER effectively achieves encrypted malicious traffic detection with the best F1 score of 0.773 and improves the F1 score of existing methods by an average of 272.5%.

==> section/authors.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}

==> table_latex/boundary.tex <==
\begin{table}[ht]
    \centering
    \caption{Data Augmentation Parameter 1: $\omega_1$, $\omega_2$}
    \label{tab:data_augmentation_minmax}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|c|c|r|r|r|r|r|r|}
            \cline{1-9}
            \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Quantity}} & \multirow{2}{*}{\textbf{Noise Ratio}} & \multicolumn{6}{|c|}{\textbf{($\omega_1$, $\omega_2$)}} \\
            \cline{4-9}
             & & & (0.3, 0.4) & (0.2, 0.4) & (0.1, 0.4) & (0.2, 0.3) & (0.1, 0.3) & (0.1, 0.2) \\
            \cline{1-9}
            \multirow{6}{*}{DoHBrw} & \multirow{6}{*}{250} 
             & 20\% & 0.752 & 0.744 & 0.740 & 0.741 & 0.736 & 0.746 \\
            \cline{3-9}
             & & 25\% & 0.721 & 0.715 & 0.720 & 0.726 & 0.721 & 0.726 \\
            \cline{3-9}
             & & 30\% & 0.715 & 0.718 & 0.720 & 0.706 & 0.717 & 0.727 \\
            \cline{3-9}
             & & 35\% & 0.715 & 0.712 & 0.721 & 0.714 & 0.727 & 0.723 \\
            \cline{3-9}
             & & 40\% & 0.717 & 0.719 & 0.718 & 0.719 & 0.717 & 0.731 \\
            \cline{3-9}
             & & 45\% & 0.714 & 0.712 & 0.724 & 0.719 & 0.725 & 0.734 \\
            \cline{1-9}
            \multirow{6}{*}{IDS+AndMal} & \multirow{6}{*}{250} 
             & 20\% & 0.787 & 0.791 & 0.800 & 0.795 & 0.787 & 0.801 \\
            \cline{3-9}
             & & 25\% & 0.795 & 0.788 & 0.777 & 0.798 & 0.781 & 0.793 \\
            \cline{3-9}
             & & 30\% & 0.790 & 0.799 & 0.794 & 0.795 & 0.797 & 0.787 \\
            \cline{3-9}
             & & 35\% & 0.792 & 0.785 & 0.775 & 0.795 & 0.779 & 0.788 \\
            \cline{3-9}
             & & 40\% & 0.777 & 0.770 & 0.779 & 0.767 & 0.779 & 0.781 \\
            \cline{3-9}
             & & 45\% & 0.766 & 0.797 & 0.791 & 0.787 & 0.782 & 0.793 \\
            \cline{1-9}
        \end{tabular}
    }
\end{table}


==> table_latex/filtering_ratio.tex <==
\begin{table}[ht]
    \centering
    \caption{Label Correction Parameter: Filtering Ratio}
    \label{tab:label_correction_arg}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|c|c|r|r|r|r|r|}
            \cline{1-8}
            \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Quantity}} & \multirow{2}{*}{\textbf{Noise Ratio}} & \multicolumn{5}{|c|}{\textbf{Filtering Ratio}} \\
            \cline{4-8}
             & & & 40\% & 45\% & 50\% & 55\% & 60\% \\
            \cline{1-8}
            \multirow{6}{*}{DoHBrw} & \multirow{6}{*}{250} 
             & 20\% & 5.17 & 3.20 & 3.20 & 3.53 & 4.00 \\
            \cline{3-8}
             & & 25\% & 5.99 & 5.46 & 3.25 & 3.57 & 4.46 \\
            \cline{3-8}
             & & 30\% & 5.48 & 3.48 & 3.64 & 3.72 & 4.44 \\
            \cline{3-8}
             & & 35\% & 6.39 & 3.17 & 2.93 & 4.06 & 5.34 \\
            \cline{3-8}
             & & 40\% & 3.60 & 4.64 & 4.36 & 4.20 & 5.56 \\
            \cline{3-8}
             & & 45\% & 4.57 & 3.31 & 3.26 & 6.28 & 9.12 \\
            \cline{1-8}
            \multirow{6}{*}{IDS+AndMal} & \multirow{6}{*}{250} 
             & 20\% & 17.27 & 16.69 & 18.00 & 17.57 & 18.55 \\
            \cline{3-8}
             & & 25\% & 16.38 & 16.92 & 17.84 & 17.87 & 18.52 \\
            \cline{3-8}
             & & 30\% & 16.50 & 17.40 & 17.89 & 17.68 & 18.50 \\
            \cline{3-8}
             & & 35\% & 16.67 & 16.70 & 17.54 & 18.15 & 18.22 \\
            \cline{3-8}
             & & 40\% & 17.05 & 17.45 & 17.83 & 17.64 & 18.45 \\
            \cline{3-8}
             & & 45\% & 16.64 & 16.87 & 17.93 & 17.75 & 18.42 \\
            \cline{1-8}
        \end{tabular}
    }
\end{table}

==> table_latex/label_correction_DoHBrw.tex <==
\begin{table}[ht]
    \centering
    \caption{Noise Ratio after label correction: DoHBrw (\%)}
    \label{tab:label_correction_DoHBrw}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|ccc}
            \toprule
            \multirow{2}{*}{\makecell[c]{Number of \\ Each Type}} & \multirow{2}{*}{\makecell[c]{Noise \\ Ratio}} & \multicolumn{3}{c}{Correction Methods}\\
             & & \textbf{Our Method} & Differential & Co-Teaching \\
            \midrule \midrule
            \multirow{6}{*}{250} 
             & 20\% & 2.46 & 6.98 & 7.30 \\
             & 25\% & 2.25 & 10.52 & 5.86 \\
             & 30\% & 2.60 & 17.64 & 5.20 \\
             & 35\% & 2.61 & 21.95 & 7.13 \\
             & 40\% & 2.40 & 30.18 & 7.66 \\
             & 45\% & 3.55 & 39.14 & 26.45 \\
            \midrule
            \multirow{6}{*}{500} 
             & 20\% & 3.84 & 6.90 & 4.02 \\
             & 25\% & 4.28 & 11.37 & 3.83 \\
             & 30\% & 4.41 & 16.97 & 5.74 \\
             & 35\% & 3.87 & 23.75 & 7.35 \\
             & 40\% & 4.34 & 30.22 & 4.55 \\
             & 45\% & 4.63 & 38.50 & 16.03 \\
            \midrule
            \multirow{6}{*}{1000} 
             & 20\% & 1.61 & 7.04 & 2.17 \\
             & 25\% & 1.99 & 12.09 & 2.33 \\
             & 30\% & 2.58 & 17.64 & 6.39 \\
             & 35\% & 4.33 & 22.67 & 6.41 \\
             & 40\% & 5.17 & 28.34 & 3.56 \\
             & 45\% & 4.04 & 37.66 & 12.07 \\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> table_latex/label_correction_IDS.tex <==
\begin{table}[ht]
    \centering
    \caption{Noise Ratio after label correction: IDS+AndMal (\%)}
    \label{tab:label_correction_IM}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|ccc}
            \cline{1-5}
            \toprule
            \multirow{2}{*}{\makecell[c]{Number of \\ Each Type}} & \multirow{2}{*}{\makecell[c]{Noise \\ Ratio}} & \multicolumn{3}{c}{Correction Methods}\\
             & & \textbf{Our Method} & Differential & Co-Teaching \\
            \midrule \midrule
            \multirow{6}{*}{250} 
             & 20\% & 18.00 & 12.25 & 23.15 \\
             & 25\% & 17.84 & 17.12 & 24.50 \\
             & 30\% & 17.89 & 21.35 & 26.30 \\
             & 35\% & 17.54 & 27.86 & 25.55 \\
             & 40\% & 17.83 & 34.65 & 28.50 \\
             & 45\% & 17.93 & 42.92 & 39.41 \\
            \midrule
            \multirow{6}{*}{500} 
             & 20\% & 17.79 & 11.05 & 19.12 \\
             & 25\% & 17.20 & 16.27 & 23.45 \\
             & 30\% & 17.60 & 21.70 & 23.10 \\
             & 35\% & 17.61 & 26.43 & 20.60 \\
             & 40\% & 17.47 & 33.53 & 19.30 \\
             & 45\% & 16.92 & 42.20 & 26.13 \\
            \midrule
            \multirow{6}{*}{1000} 
             & 20\% & 17.64 & 11.62 & 16.22 \\
             & 25\% & 17.32 & 16.26 & 20.76 \\
             & 30\% & 17.28 & 20.55 & 22.54 \\
             & 35\% & 17.20 & 24.98 & 16.97 \\
             & 40\% & 16.16 & 31.40 & 16.62 \\
             & 45\% & 17.19 & 39.50 & 23.10 \\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> table_latex/little_noise.tex <==
\begin{table*}[ht]
    \centering
    \caption{The F1-score with few-noise training set (Training Size: 500)}
    \label{tab:detection_f1_little_noise}
    \resizebox{0.9\textwidth}{!}{
        \begin{tabular}{c|c|cccccc|cc|c}
            \toprule
            \multirow{2}{*}{\makecell[c]{\textbf{Noise} \\ \textbf{Ratio}}} & \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{\textbf{Detection Methods Based on FS}} & \multicolumn{2}{c|}{\textbf{Based on ETA}} & \multirow{2}{*}{\textbf{Ours}} \\
             & & \textbf{FS} & \textbf{Co+FS} & \textbf{DT+FS} & \textbf{ODDS+FS} & \textbf{SMOTE+FS} & \textbf{DT+ODDS+FS} & \textbf{ETA} & \textbf{DT+ODDS+ETA} \\
            \midrule 
            \multirow{3}{*}{0\%} 
 & DoHBrw & .62 $\pm$ .00 & .38 $\pm$ .00 & .65 $\pm$ .12 & .90 $\pm$ .01 & .77 $\pm$ .06 & .63 $\pm$ .12 & .85 $\pm$ .21 & .59 $\pm$ .24 & .74 $\pm$ .03 \\
 & IDS  &  .76 $\pm$ .03 & .15 $\pm$ .06 & .54 $\pm$ .05 & .61 $\pm$ .03 & .43 $\pm$ .04 & .58 $\pm$ .05 & .98 $\pm$ .00 & .88 $\pm$ .05 & .79 $\pm$ .02 \\
 & IDS/DoH& .78 $\pm$ .02 & .18 $\pm$ .04 & .57 $\pm$ .03 & .61 $\pm$ .10 & .41 $\pm$ .03 & .56 $\pm$ .05 & .98 $\pm$ .00 & .90 $\pm$ .06 & .85 $\pm$ .03 \\
            \midrule
            \multirow{3}{*}{10\%} 
 & DoHBrw & .61 $\pm$ .05 & .30 $\pm$ .07 & .85 $\pm$ .14 & .92 $\pm$ .05 & .80 $\pm$ .15 & .83 $\pm$ .17 & .55 $\pm$ .23 & .44 $\pm$ .10 & .71 $\pm$ .07 \\
 & IDS & .68 $\pm$ .06 & .58 $\pm$ .27 & .75 $\pm$ .09 & .73 $\pm$ .11 & .44 $\pm$ .08 & .72 $\pm$ .10 & .80 $\pm$ .17 & .75 $\pm$ .12 & .76 $\pm$ .03 \\
 & IDS/DoH & .67 $\pm$ .08 & .78 $\pm$ .08 & .75 $\pm$ .07 & .76 $\pm$ .07 & .44 $\pm$ .07 & .75 $\pm$ .10 & .76 $\pm$ .22 & .73 $\pm$ .20 & \textbf{.86} $\pm$ .02 \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> table_latex/multiplier.tex <==
\begin{table}[ht]
    \centering
    \caption{Data Augmentation Parameter 2: multiplier}
    \label{tab:data_augmentation_multi}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|c|c|r|r|r|r|r|}
            \cline{1-8}
            \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Quantity}} & \multirow{2}{*}{\textbf{Noise Ratio}} & \multicolumn{5}{|c|}{\textbf{multiplier}} \\
            \cline{4-8}
             & & & 2 & 4 & 5 & 6 & 8 \\
            \cline{1-8}
            \multirow{6}{*}{DoHBrw} & \multirow{6}{*}{250} 
             & 20\% & 0.772 & 0.772 & 0.778 & 0.771 & 0.776 \\
            \cline{3-8}
             & & 25\% & 0.774 & 0.776 & 0.780 & 0.775 & 0.771 \\
            \cline{3-8}
             & & 30\% & 0.772 & 0.780 & 0.779 & 0.777 & 0.770 \\
            \cline{3-8}
             & & 35\% & 0.773 & 0.779 & 0.778 & 0.771 & 0.774 \\
            \cline{3-8}
             & & 40\% & 0.774 & 0.772 & 0.774 & 0.766 & 0.769 \\
            \cline{3-8}
             & & 45\% & 0.769 & 0.780 & 0.770 & 0.764 & 0.778 \\
            \cline{1-8}
            \multirow{6}{*}{IDS+AndMal} & \multirow{6}{*}{250} 
             & 20\% & 0.820 & 0.815 & 0.821 & 0.808 & 0.821 \\
            \cline{3-8}
             & & 25\% & 0.819 & 0.823 & 0.822 & 0.817 & 0.810 \\
            \cline{3-8}
             & & 30\% & 0.823 & 0.817 & 0.822 & 0.824 & 0.821 \\
            \cline{3-8}
             & & 35\% & 0.820 & 0.827 & 0.813 & 0.819 & 0.816 \\
            \cline{3-8}
             & & 40\% & 0.819 & 0.817 & 0.831 & 0.819 & 0.815 \\
            \cline{3-8}
             & & 45\% & 0.826 & 0.825 & 0.822 & 0.821 & 0.827 \\
            \cline{1-8}
        \end{tabular}
    }
\end{table}

==> table_latex/precision_recall_DoHBrw.tex <==
\begin{table*}[ht]
    \centering
    \caption{(Recall, Prec) of each detection model on the DoHBrw dataset}
    \label{tab:detection_precision_recall_DoHBrw}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|ccccccc|cc}
            \toprule
            \multirow{2}{*}{\makecell[c]{Number of \\ Each Type}} & \multirow{2}{*}{\makecell[c]{Noise \\ Ratio}} & \multirow{2}{*}{\makecell[c]{Our \\ Method}} & \multicolumn{6}{c|}{Detection Methods Based on FS} & \multicolumn{2}{c}{Based on ETA} \\
             & & & FS & Co+FS & DT+FS & ODDS+FS & SMOTE+FS & DT+ODDS+FS & ETA & DT+ODDS+ETA \\
            \midrule \midrule
            \multirow{6}{*}{250} 
             & 20\% & \textbf{(0.96, 0.65)} & (0.32, 0.79) & (0.44, 0.75) & (0.50, 0.51) & (0.14, 0.69) & (1.00, 0.50) & (0.47, 0.66) & (1.00, 0.55) & (1.00, 0.54) \\
             & 25\% & \textbf{(0.98, 0.65)} & (0.36, 0.79) & (0.33, 0.70) & (0.61, 0.56) & (0.06, 0.71) & (1.00, 0.50) & (0.51, 0.68) & (1.00, 0.54) & (1.00, 0.54) \\
             & 30\% & \textbf{(0.96, 0.66)} & (0.29, 0.80) & (0.40, 0.66) & (0.53, 0.59) & (0.10, 0.88) & (1.00, 0.50) & (0.49, 0.67) & (1.00, 0.54) & (1.00, 0.54) \\
             & 35\% & \textbf{(0.96, 0.66)} & (0.30, 0.72) & (0.43, 0.65) & (0.52, 0.48) & (0.03, 0.97) & (0.99, 0.50) & (0.44, 0.67) & (0.90, 0.63) & (1.00, 0.54) \\
             & 40\% & \textbf{(0.96, 0.65)} & (0.31, 0.63) & (0.53, 0.57) & (0.41, 0.44) & (0.04, 0.71) & (0.98, 0.50) & (0.35, 0.62) & (0.59, 0.85) & (0.79, 0.52) \\
             & 45\% & \textbf{(0.96, 0.64)} & (0.29, 0.47) & (0.58, 0.47) & (0.34, 0.52) & (0.02, 0.66) & (0.97, 0.50) & (0.40, 0.55) & (0.59, 0.93) & (0.49, 0.37) \\
            \midrule
            \multirow{6}{*}{500} 
             & 20\% & \textbf{(0.87, 0.75)} & (0.49, 0.75) & (0.49, 0.71) & (0.57, 0.46) & (0.14, 0.79) & (1.00, 0.51) & (0.55, 0.68) & (1.00, 0.60) & (0.94, 0.53) \\
             & 25\% & \textbf{(0.91, 0.69)} & (0.42, 0.73) & (0.44, 0.71) & (0.56, 0.55) & (0.12, 0.74) & (1.00, 0.50) & (0.62, 0.69) & (0.94, 0.65) & (1.00, 0.54) \\
             & 30\% & \textbf{(0.90, 0.70)} & (0.40, 0.73) & (0.48, 0.69) & (0.50, 0.48) & (0.06, 0.81) & (0.99, 0.50) & (0.58, 0.63) & (0.63, 1.00) & (0.73, 0.54) \\
             & 35\% & \textbf{(0.86, 0.72)} & (0.39, 0.64) & (0.49, 0.64) & (0.52, 0.53) & (0.05, 0.84) & (0.99, 0.50) & (0.29, 0.66) & (0.49, 1.00) & (0.49, 0.70) \\
             & 40\% & \textbf{(0.91, 0.68)} & (0.42, 0.56) & (0.56, 0.58) & (0.59, 0.41) & (0.02, 0.61) & (0.98, 0.50) & (0.37, 0.56) & (0.49, 1.00) & (0.55, 0.68) \\
             & 45\% & \textbf{(0.92, 0.71)} & (0.45, 0.55) & (0.63, 0.49) & (0.32, 0.45) & (0.01, 0.47) & (0.96, 0.50) & (0.34, 0.54) & (0.69, 0.81) & (0.84, 0.55) \\
            \midrule
            \multirow{6}{*}{1000} 
             & 20\% & \textbf{(0.87, 0.72)} & (0.44, 0.64) & (0.43, 0.65) & (0.53, 0.67) & (0.21, 0.81) & (1.00, 0.51) & (0.67, 0.50) & (1.00, 0.55) & (1.00, 0.54) \\
             & 25\% & \textbf{(0.94, 0.66)} & (0.64, 0.75) & (0.55, 0.74) & (0.51, 0.57) & (0.09, 0.89) & (1.00, 0.51) & (0.74, 0.52) & (1.00, 0.55) & (1.00, 0.55) \\
             & 30\% & \textbf{(0.91, 0.69)} & (0.61, 0.68) & (0.47, 0.76) & (0.54, 0.54) & (0.04, 0.71) & (1.00, 0.50) & (0.76, 0.45) & (1.00, 0.55) & (1.00, 0.55) \\
             & 35\% & \textbf{(0.95, 0.65)} & (0.61, 0.58) & (0.60, 0.70) & (0.40, 0.59) & (0.03, 0.97) & (0.99, 0.50) & (0.69, 0.51) & (1.00, 0.55) & (1.00, 0.55) \\
             & 40\% & \textbf{(0.95, 0.65)} & (0.63, 0.58) & (0.56, 0.63) & (0.54, 0.52) & (0.02, 0.63) & (0.98, 0.50) & (0.59, 0.50) & (1.00, 0.55) & (1.00, 0.55) \\
             & 45\% & \textbf{(0.95, 0.65)} & (0.65, 0.55) & (0.68, 0.59) & (0.31, 0.57) & (0.02, 0.58) & (0.97, 0.50) & (0.56, 0.56) & (0.49, 1.00) & (0.49, 0.87) \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> table_latex/precision_recall_IDS_AndMal.tex <==
\begin{table*}[ht]
    \centering
    \caption{(Recall, Prec) of each detection model on the IDS dataset}
    \label{tab:detection_precision_recall_IM}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c|ccccccc|cc}
            \toprule
            \multirow{2}{*}{\makecell[c]{Number of \\ Each Type}} & \multirow{2}{*}{\makecell[c]{Noise \\ Ratio}} & \multirow{2}{*}{\makecell[c]{Our \\ Method}} & \multicolumn{6}{c|}{Detection Methods Based on FS} & \multicolumn{2}{c}{Based on ETA} \\
             & & & FS & Co+FS & DT+FS & ODDS+FS & SMOTE+FS & DT+ODDS+FS & ETA & DT+ODDS+ETA \\
            \midrule \midrule
            \multirow{6}{*}{250} 
             & 20\% & \textbf{(0.73, 0.82)} & (0.88, 0.14) & (0.82, 0.45) & (0.85, 0.23) & (0.09, 0.92) & (0.99, 0.03) & (0.48, 0.82) & (0.96, 0.35) & (0.96, 0.25) \\
             & 25\% & \textbf{(0.72, 0.75)} & (0.86, 0.10) & (0.86, 0.31) & (0.89, 0.17) & (0.02, 0.79) & (0.99, 0.04) & (0.27, 0.65) & (0.84, 0.29) & (0.88, 0.29) \\
             & 30\% & \textbf{(0.70, 0.84)} & (0.90, 0.08) & (0.81, 0.37) & (0.89, 0.13) & (0.02, 0.45) & (0.98, 0.03) & (0.31, 0.73) & (0.84, 0.33) & (0.84, 0.26) \\
             & 35\% & \textbf{(0.70, 0.85)} & (0.81, 0.06) & (0.83, 0.38) & (0.82, 0.18) & (0.02, 0.75) & (0.99, 0.03) & (0.24, 0.78) & (0.64, 0.20) & (0.67, 0.21) \\
             & 40\% & \textbf{(0.69, 0.75)} & (0.77, 0.05) & (0.83, 0.19) & (0.80, 0.10) & (0.02, 0.05) & (0.99, 0.03) & (0.10, 0.60) & (0.72, 0.16) & (0.76, 0.16) \\
             & 45\% & \textbf{(0.72, 0.79)} & (0.51, 0.03) & (0.50, 0.53) & (0.76, 0.07) & (0.01, 0.32) & (0.99, 0.03) & (0.11, 0.58) & (0.76, 0.11) & (0.66, 0.05) \\
            \midrule
            \multirow{6}{*}{500} 
             & 20\% & \textbf{(0.70, 0.76)} & (0.93, 0.12) & (0.87, 0.34) & (0.89, 0.24) & (0.02, 0.86) & (0.99, 0.03) & (0.26, 0.70) & (0.87, 0.37) & (0.89, 0.35) \\
             & 25\% & \textbf{(0.69, 0.91)} & (0.94, 0.11) & (0.85, 0.45) & (0.90, 0.20) & (0.02, 0.82) & (0.99, 0.03) & (0.42, 0.81) & (0.90, 0.31) & (0.92, 0.37) \\
             & 30\% & \textbf{(0.70, 0.77)} & (0.94, 0.08) & (0.83, 0.43) & (0.91, 0.16) & (0.04, 0.90) & (0.99, 0.03) & (0.33, 0.74) & (0.78, 0.44) & (0.85, 0.41) \\
             & 35\% & \textbf{(0.70, 0.85)} & (0.86, 0.06) & (0.84, 0.34) & (0.90, 0.12) & (0.02, 0.70) & (0.99, 0.03) & (0.21, 0.71) & (0.66, 0.45) & (0.77, 0.26) \\
             & 40\% & \textbf{(0.70, 0.73)} & (0.74, 0.05) & (0.81, 0.18) & (0.80, 0.16) & (0.02, 0.40) & (1.00, 0.03) & (0.19, 0.51) & (0.74, 0.23) & (0.71, 0.15) \\
             & 45\% & \textbf{(0.69, 0.93)} & (0.71, 0.04) & (0.71, 0.13) & (0.69, 0.07) & (0.03, 0.05) & (1.00, 0.03) & (0.12, 0.60) & (0.62, 0.22) & (0.79, 0.26) \\
            \midrule
            \multirow{6}{*}{1000} 
             & 20\% & \textbf{(0.70, 0.95)} & (0.93, 0.16) & (0.88, 0.40) & (0.91, 0.31) & (0.13, 0.89) & (0.99, 0.03) & (0.53, 0.71) & (0.92, 0.47) & (0.94, 0.39) \\
             & 25\% & \textbf{(0.73, 0.82)} & (0.92, 0.12) & (0.89, 0.33) & (0.92, 0.26) & (0.05, 0.79) & (0.99, 0.03) & (0.45, 0.90) & (0.99, 0.49) & (0.99, 0.47) \\
             & 30\% & \textbf{(0.73, 0.77)} & (0.85, 0.11) & (0.88, 0.33) & (0.92, 0.20) & (0.03, 0.75) & (1.00, 0.03) & (0.39, 0.96) & (0.80, 0.49) & (0.81, 0.47) \\
             & 35\% & \textbf{(0.73, 0.77)} & (0.81, 0.07) & (0.86, 0.31) & (0.90, 0.18) & (0.02, 0.77) & (0.99, 0.03) & (0.37, 0.87) & (0.73, 0.40) & (0.77, 0.40) \\
             & 40\% & \textbf{(0.70, 0.79)} & (0.74, 0.06) & (0.87, 0.28) & (0.90, 0.11) & (0.02, 0.71) & (1.00, 0.03) & (0.17, 0.67) & (0.77, 0.35) & (0.77, 0.29) \\
             & 45\% & \textbf{(0.70, 0.69)} & (0.38, 0.04) & (0.66, 0.15) & (0.86, 0.08) & (0.01, 0.56) & (1.00, 0.03) & (0.17, 0.47) & (0.64, 0.25) & (0.68, 0.25) \\
            \bottomrule
        \end{tabular}
    }
\end{table*}
